Lower Quantity, Higher Quality: Auditing News Content and User Perceptions on Twitter/X Algorithmic versus Chronological Timelines

Social media personalization algorithms increasingly influence the flow of civic information through society, resulting in concerns about "filter bubbles", "echo chambers", and other ways they might exacerbate ideological segregation and fan the spread of polarizing content. To address these concerns, we designed and conducted a sociotechnical audit (STA) to investigate how Twitter/X's timeline algorithm affects news curation while also tracking how user perceptions change in response. We deployed a custom-built system that, over the course of three weeks, passively tracked all tweets loaded in users' browsers in the first week, then in the second week enacted an intervention to users' Twitter/X homepage to restrict their view to only the algorithmic or chronological timeline (randomized). We flipped this condition for each user in the third week. We ran our audit in late 2023, collecting user-centered metrics (self-reported survey measures) and platform-centered metrics (views, clicks, likes) for 243 users, along with over 800,000 tweets. Using the STA framework, our results are two-fold: (1) Our algorithm audit finds that Twitter/X's algorithmic timeline resulted in a lower quantity but higher quality of news -- less ideologically congruent, less extreme, and slightly more reliable -- compared to the chronological timeline. (2) Our user audit suggests that although our timeline intervention had significant effects on users' behaviors, it had little impact on their overall perceptions of the platform. Our paper discusses these findings and their broader implications in the context of algorithmic news curation, user-centric audits, and avenues for independent social science research.

==> sections/cuts.tex <==
% In terms of differences along partisan lines, on the \Algo timeline of right-leaning accounts, 40.6\% of all news links were from right-leaning news domains and 11.8\% were from left-leaning news domains. On the \Algo timeline of left-leaning accounts, 38.7\% of all news links were from left-leaning news domains and 2.7\% were from right-leaning news domains. On the \Chrono timeline of right-leaning accounts, 19.7\% of all news links were from right-leaning news domains and 13.5\% were from left-leaning news domains. On the \Chrono timeline of left-leaning accounts, 19.8\% of all news links were from left-leaning news domains and 1.5\% were from right-leaning news domains. 

% \begin{table}
%   \caption{Participant-level averages and standard deviations for key metrics across different \Twitter surfaces during the observation week.}
%   \label{tab:observation-freq}
% \begin{tabular}{lllllll}
% \toprule
%                               & \multicolumn{2}{l}{Algorithmic} & \multicolumn{2}{l}{Chronological} & \multicolumn{2}{l}{Non-timeline} \\
%                               \midrule
%                               & Mean & SD & Mean & SD & Mean & SD \\
%                               \midrule
% Number of tweets seen         & 557 & 1546 & 406 & 547 & 787 & 1546 \\
% Number of tweet engagements   & 40.6 & 141 & 7.32 & 10.7 & 25.8 & 57.8 \\
% % Number of tweets seen with links      &                 &               &                  &                &                &              \\
% % Number of tweets seen with news links & 18.6 & 49.5 & 44.3 & 100 & 13.7 & 33 \\
% \bottomrule
% \end{tabular}
% \end{table}

% \begin{table}
%   \caption{Percentage of tweets containing URLs and news URLs  across different \Twitter surfaces during the observation week.}
%   \label{tab:observation-perc}
% \begin{tabular}{llll}
% \toprule
%                              & Algorithmic & Chronological & Non-timeline \\
%                              \midrule
% \% of URLs      &      &        &              \\
% \% of news URLs & 1.26 & 5.47 & 0.65 \\
% \bottomrule
% \end{tabular}
% \end{table}

\section{Method}

% \begin{table}
%   \caption{Number of participants in each condition}
%   \label{tab:freq}
%   \begin{tabular}{llll}
%     \toprule
%     Phase    & Ideology & Algorithmic & Chronological \\
%     \midrule
%                  Intervention 1 & Left   & 80          & 78            \\
%                                 & Middle & 16          & 19            \\
%                                 & Right  & 27          & 23            \\
%     \midrule
%                  Intervention 2 & Left   & 74          & 76            \\
%                                 & Middle & 15          & 14            \\
%                                 & Right  & 23          & 26            \\
%     \bottomrule
%    \end{tabular}
% \end{table}


% \subsection{Analysis models}


\section{Related Work}
% Despite industrial support contributing to the scholarly understanding of platform algorithms, criticism arises regarding the restricted research independence , which hinders valid replication of the results. Besides, for most researchers outside of tech companies, the platform-controlled data is not always accessible. For instance, Twitter/X auditors recruited crowdsourcing users and scraped metrics data using platform APIs \cite{milli_twitters_nodate}, which, however, is no longer feasible given the deepened platform restrictions these days \cite{freelon_computational_2018,davidson_platform-controlled_2023}. 

% Specifically, researchers invited opt-in crowdsourcing workers to install browser extensions to their own devices, and automatically collected visible URLs \cite{Lam_2023} or HTML snapshots \cite{robertson_users_2023} within the range of browser viewport from backstage operations, which would be ecologically valid exposure data (i.e., what people indeed see on the platform during a given period). Also, these studies work around the data restrictions of platforms by obtaining consent from end users, which paves new ways for user-involved algorithm audits.

% \subsubsection{Summary}
% algorithm-centric to user-centric: sociotechnical audit
This section reviews the dominant methods used by platform auditors. Motivated by previous studies auditing real-world user behaviors in online ecosystems and collecting data through independent approaches \cite{robertson_users_2023, Lam_2023}, we design the current study by leveraging crowdsourcing workers and scraping users' activity data on Twitter/X with consent. We believe this methodology decision would benefit the study in the following aspects: First, we can customize the experimental intervention through external software and make causal inferences from the results. Second, we can make user-centric evaluations such that users are affected under different algorithmic conditions\cite{Lam_2023}. Third, we independently collect the valid behavioral data observed during the study solely under the permission of participants. 

% Relying on large-scale sock puppet accounts, auditors found a consistent tendency for YouTube algorithms to recommend congenial videos to users\cite{haroon_auditing_2023}. Moreover, researchers found that Facebook's algorithms increased exposure to both cross-cutting and like-minded sources\cite{guess_how_2023}, indicating that news diversity and ideological congruence are not exclusive consequences. 

% Notably, depending on operation purposes, algorithm audits of different organizations may generate different results \cite{bandy_review_2021}. 

For Twitter/X specifically, existing research provides mixed results. While some showed that algorithmic curation did not amplify far-left or far-right sources \cite{huszar_algorithmic_2022}, others found that personalization algorithms amplified emotional content with anger and outgroup animosity\cite{milli_twitters_nodate}. These results indicate that whether Twitter/X algorithms prioritize exposure to extreme news remains to be an open question. Based on previous evidence on other platforms, we hypothesize that Twitter/X algorithms have a similar effect and tend to favor extreme news sources.


\section{Method}

% By pairing our data collection with participant behavior traces and surveys, we are able to identify and study the Tweets that participants are exposed to and ask 
% We instantiate our method By recruiting real-world users and observing their beh
%  "a two-part audit of a sociotechnical system that consists of both an Algorithm Audit and a User Audit. We define Algorithm Audits as investigations that change inputs to an algorithmic system (e.g., testing for a range of users or behaviors) and observe the system’s outputs to infer properties of the system. Meanwhile, we define User Audits as investigations that change inputs to the user (e.g., different system outputs) and observe their effects to draw conclusions about users." \cite{Lam_2023} 

% The benefit of switch: a within-subject design: but need to test the order effects (t.test(week 2 for you group & week 3 for you group) p>0.05)

% Control for Individual Differences: By having participants serve as their own controls, you can reduce the impact of individual differences that may affect the results. This is particularly valuable when dealing with small sample sizes.

% Increased Statistical Power: Since participants are exposed to both conditions, the design can potentially increase statistical power by reducing the variability associated with individual differences.

% Time-Related Effects: The design allows you to examine how the effects of the interventions change over time within the same individuals.

% Enhanced Internal Validity: The switching of conditions helps control for extraneous variables and strengthens the internal validity of your study.

% However, it's essential to be cautious and consider potential order effects, carryover effects, or other confounding factors that might arise from the switching of conditions. Proper counterbalancing and randomization techniques can help address some of these concerns.

\section{Results}

% \begin{itemize}
%     \item How many tweets people see on average, 
%     \item (breakdown of number of tweets with links and what percentage of links are news)
%     \item how much news they see
%     \item (report numbers in line and by demographic/ideology groups breakdown figure goes to supplementary). 
%     \item how slanted and reliable the news they see is. (Overall population, democrats, republicans)
%     \item overall time spend on Twitter; duration and engagement 
%    % exploratory findings
%     \item People get a lot of tweets outside of the timeline.
%     \item User agency in switching between for you and following?
%     \item The top external news sites were
% \end{itemize}



% For You is better than Following:
% \begin{itemize}
%     \item People spend slightly more time on it 
%     \item They do see more news on Following, but... 
%     \item They engage less with those news tweets
%     \item They see less self-congruent news on For You (greater diversity) 
%     \item They see less extreme news on FY
%     \item Same reliability (maybe even a little higher on FY)
%     \item Survey: People can't tell the difference (they like them both the same, no big difference in ppl's perception)
% \end{itemize}
% Conservatives see more unreliable news regardless of condition 
% Stronger partisans see more congruent content regardless of condition
% Survey: people always think Twitter algo is biased against them 


%\subsubsection{RQ1: How does algorithmic timeline curation affect Twitter users' information behaviors on their home timeline?}
%\begin{itemize}
%\item People see more tweets on for you than following timeline (M=224.8, SE=60.9, p<0.001).
%\item People spent more time on tweets on the for you timeline than following (M=0.709, SE=0.21, p<0.003).
%\item People engage slightly but significantly more with tweets when they are in for you than in following (M=0.01, SE=0.0007, p<0.0001). At the user level of analysis, users on average engaged with more tweets on For you than following timeline (M=14.47, SE=4.95, p<0.05).
% \item People visit other social media sites more (N of visits/time spend on other sites) \dm{in which condition}
%\end{itemize}

%\subsubsection{RQ3: How does algorithmic timeline curation affect Twitter users’ news behaviors on their home timeline?}
%\begin{itemize}
%\item People see more news tweets on following than for you. On average people saw 42.1 more news tweets on following than for you (SD=11.7, p < 0.001) number\_of\_tweets ~ user\_condition+ (1|user\_id). 
%\item People spend a longer time on following than for you [Need to verify]
%\item But people engaged slightly more with news tweets on For you than on following (p < .0001).   
%\item News slant based on Ad Fontes: for you vs. following. The mean absolute bias is greater for Following than For you by 1.3 (p < 0.005).
%\item News reliability based on Ad Fontes: for you vs. following. Users see more reliable news in Following than in For you, on average 1.3 higher reliability (p < .0001).
%\end{itemize}

% \begin{itemize}
% \item Do users who see more conservative/liberal tweets adjust their responses to own\_timeline questions? Yes when reading conservative/ liberal news, people do report seeing such changes (p < 0.001).
% \item No, people when reading more or less conservative/liberal news don't change their perception about "what news are available on Twitter for all users"
% \item negative and significant; People when reading more conservative news think the timelines of Republicans are not THAT conservative
% \item People when reading more liberal news think the timelines of Democrats are more liberal
% \item (Need to reexamine the news credibility and news trust.) disconnect between perception and what they actually see. Note: a vibe
% \item mean\_bias/median\_bias does not matter: what people see does not change their perception of Twitter algorithm's bias. Hostile media effect (HME).
% \item congruence does not change neutral\_algo responses for within-person comparisons


% \begin{table}
%   \caption{Averages and standard deviations for survey measures for Survey 2 (after observation period).}
%   \label{tab:survey-summary-statistics}
% \begin{tabular}{lllllll}
% \toprule
%                               & \multicolumn{2}{l}{Democrat} & \multicolumn{2}{l}{Independent} & \multicolumn{2}{l}{Republican} \\
%                               \midrule
%                               & Mean & SD & Mean & SD & Mean & SD \\
%                               \midrule
% % Perceived Polarization Own Timeline         & 36.83 & 24.82 & 45.68 & 27.91 & 63.95 & 20.77 \\
% % Perceived Polarization Overall   & 53.20 & 20.19 & 53.51 & 18.39 & 50.91 & 17.82 \\
% % Perceived Polarization Rep Timeline   & 82.00 & 20.37 & 74.06 & 17.21 & 69.17 & 18.48 \\
% % Perceived Polarization Dem Timeline   & 25.77 & 19.24 & 31.65 & 22.34 & 27.86 & 23.67 \\
% Satisfaction User Experience   & 40.6 & 141 & 7.32 & 10.7 & 25.8 & 57.8 \\
% % Satisfaction News   & 2.79 & 1.10 & 3.06 & 0.92 & 3.82 & 0.91 \\
% % Perceived News Credibility   & 2.75 & 0.95 & 3.03 & 0.86 & 3.46 & 0.91 \\
% % News Trust   & 2.85 & 1.04 & 2.96 & 0.98 & 3.53 & 0.86 \\
% Perceived Neutrality of Platform   & 3.55 & 1.03 & 3.51 & 0.73 & 2.97 & 0.69 \\
% % Support for Regulation   & 3.10 & 1.27 & 2.27 & 1.30 & 1.93 & 1.26 \\
% Recommendation Algorithm Awareness   & 40.6 & 141 & 7.32 & 10.7 & 25.8 & 57.8 \\
% Awareness of Algorithm Prioritizing Content   & 40.6 & 141 & 7.32 & 10.7 & 25. 8 & 57.8 \\
% Awareness of Algorithm Tailoring Content   & 40.6 & 141 & 7.32 & 10.7 & 25.8 & 57.8 \\
% % Awareness of Algorithm Delivering Different News   & 4.12 & 0.98 & 3.68 & 1.31 & 4.02 & 0.94 \\
% % Algorithms Distort Online News  & 3.96 & 0.86 & 3.58 & 0.98 & 3.64 & 1.00 \\
% % Democracy Harmed by Algorithm-delivered News  & 3.23 & 1.07 & 2.82 & 1.07 & 2.60 & 1.11 \\
% % Algorithm-delivered News Slanted Against My Views  & 2.79 & 1.06 & 3.03 & 0.86 & 3.02 & 0.91 \\
% \bottomrule
% \end{tabular}
% \end{table}
